Relax and penalize: a new bilevel approach to mixed-binary hyperparameter optimization

In recent years, bilevel approaches have become very popular to efficiently estimate high-dimensional hyperparameters of machine learning models. However, to date, binary parameters are handled by continuous relaxation and rounding strategies, which could lead to inconsistent solutions. In this context, we tackle the challenging optimization of mixed-binary hyperparameters by resorting to an equivalent continuous bilevel reformulation based on an appropriate penalty term. We propose an algorithmic framework that, under suitable assumptions, is guaranteed to provide mixed-binary solutions. Moreover, the generality of the method allows to safely use existing continuous bilevel solvers within the proposed framework. We evaluate the performance of our approach for two specific machine learning problems, i.e., the estimation of the group-sparsity structure in regression problems and the data distillation problem. The reported results show that our method is competitive with state-of-the-art approaches based on relaxation and rounding

==> data/distinf.tex <==
\pgfplotstableread{
y x
0.893903461242812 1
0.894189491130417 101
0.894245562488453 201
0.894212695651189 301
0.894396388097988 401
0.894476616479533 501
0.894559738261505 601
0.894880524354015 701
0.895017955763558 801
0.89518039355622 901
0.895583506826112 1001
0.895879718618502 1101
0.895822647650221 1201
0.896292092111924 1301
0.896621087457957 1401
0.896875339326022 1501
0.897006394581998 1601
0.897258037595848 1701
0.897430190211469 1801
0.897478391979445 1901
0.897630955286602 2001
0.897598356381032 2101
0.897733285718285 2201
0.897835255106821 2301
0.898020138600356 2401
0.898279696995113 2501
0.898344053978833 2601
0.898223729328601 2701
0.89806561029474 2801
0.897914630100504 2901
0.897738676052507 3001
0.897598333248633 3101
0.897439213505239 3201
0.897317971328148 3301
0.897187663574347 3401
0.89724079480322 3501
0.897081745143099 3601
0.897308689414971 3701
0.897147080802317 3801
0.897082444655967 3901
0.89701454385747 4001
0.896892067038344 4101
0.896765284803669 4201
0.896631997405571 4301
0.89654680782514 4401
0.896382920561195 4501
0.89614117316124 4601
0.895899304721958 4701
0.89561654818512 4801
0.895194552790565 4901
0.894971865497418 5001
0.894680289702065 5101
0.894515739796958 5201
0.894261240773329 5301
0.894055853721544 5401
0.89383210152873 5501
0.893640376701861 5601
0.893424295181115 5701
0.893101371594873 5801
0.892882902414164 5901
0.892672179789698 6001
0.892395876201626 6101
0.892296202250319 6201
0.89209716106489 6301
0.891733619017532 6401
0.891449288346539 6501
0.891263293263798 6601
0.89096477400141 6701
0.890786377658492 6801
0.890480729909875 6901
0.890119544699263 7001
0.889912324124775 7101
0.889431145874127 7201
0.889252433731445 7301
0.888741650643313 7401
0.888424448474385 7501
0.887821400617184 7601
0.887200868447057 7701
0.886238590835511 7801
0.885541240779235 7901
0.884997316696679 8001
0.884528285704779 8101
0.883683951323311 8201
0.882625644010135 8301
0.882320936483198 8401
0.881455728030721 8501
0.880265065242885 8601
0.879875093267379 8701
0.879251156834294 8801
0.879158168228821 8901
0.878140182824569 9001
0.876866851422044 9101
0.876375175235985 9201
0.875728599810965 9301
0.874232652830999 9401
0.873126581974786 9501
0.872089240017285 9601
0.870802424793787 9701
0.868776121486347 9801
0.866042866686098 9901
0.862628796707654 10001
0.859712659932273 10101
0.856967203611566 10201
0.855861810896048 10301
0.853340117226381 10401
0.850930908908213 10501
0.848505153232806 10601
0.846024730453052 10701
0.842855770180863 10801
0.83929214175508 10901
0.835410097993251 11001
0.831430914917902 11101
0.828960013713882 11201
0.82548727026577 11301
0.82007802815269 11401
0.816495910072236 11501
0.812786266336932 11601
0.808464604871545 11701
0.8036595396569 11801
0.798963874275801 11901
0.793092122962764 12001
0.789007922775368 12101
0.784653363672717 12201
0.780018917922712 12301
0.774856300731737 12401
0.770687267141191 12501
0.768869664810254 12601
0.766321033370611 12701
0.763509614532649 12801
0.763201116382895 12901
0.760693684447867 13001
0.75433467284817 13101
0.747657479169779 13201
0.740993164142862 13301
0.734258922142575 13401
0.726230705830413 13501
0.718209227821674 13601
0.709653696537592 13701
0.700171122335672 13801
0.691104335407091 13901
0.680232638637476 14001
0.675054771869559 14101
0.668515196852137 14201
0.662004690972913 14301
0.65561214362482 14401
0.649275624008046 14501
0.643616936450214 14601
0.637856593186333 14701
0.632825669778245 14801
0.625010252746811 14901
0.619714911462672 15001
0.61267813860715 15101
0.605314987975885 15201
0.598957865413071 15301
0.592883922936106 15401
0.587859872836531 15501
0.581714184290888 15601
0.577137479043928 15701
0.573248606238535 15801
0.570226981272497 15901
0.567916470788393 16001
0.564173312074045 16101
0.562732997327017 16201
0.560064015269276 16301
0.555859666473543 16401
0.553016781424225 16501
0.550041783264281 16601
0.547197997367236 16701
0.544627352443986 16801
0.541232042415028 16901
0.538631442046082 17001
0.536812067988085 17101
0.534886446351736 17201
0.533842013045245 17301
0.533339523849995 17401
0.53258213876256 17501
0.530632473442526 17601
0.528364149864579 17701
0.526679835501118 17801
0.525043108441232 17901
0.523551393730889 18001
0.522265689729452 18101
0.522117162361797 18201
0.521470049000896 18301
0.518976934526585 18401
0.517225029349586 18501
0.515019494948187 18601
0.523664300647453 18701
0.523487857723528 18801
0.508680356525302 18901
0.507644319527951 19001
0.506763901813595 19101
0.504947570203739 19201
0.502923529432419 19301
0.500908292148785 19401
0.499651852313076 19501
0.498511260868185 19601
0.498170338134786 19701
0.49790618486884 19801
0.497640667498385 19901
0.497412373980991 20001
0.49701970317268 20101
0.496838824086248 20201
0.496547607419543 20301
0.498427301743771 20401
0.495828018888223 20501
0.495331461661755 20601
0.495311855488891 20701
0.495073458131351 20801
0.494267551931053 20901
0.493876076103069 21001
0.493252740264864 21101
0.492967715155818 21201
0.492291107662467 21301
0.491362096622242 21401
0.490663946120755 21501
0.489906906042728 21601
0.49216865817651 21701
0.498684343726809 21801
0.497812796174303 21901
0.492739206124663 22001
0.491651500274607 22101
0.49372817259599 22201
0.497557153102305 22301
0.498486906451624 22401
0.494348681139057 22501
0.489848958652371 22601
0.488264834721878 22701
0.488593039919316 22801
0.488934436187953 22901
0.48874099142327 23001
0.488407875915075 23101
0.488236493042154 23201
0.487428016437612 23301
0.487454147411046 23401
0.489657924399896 23501
0.491330121617353 23601
0.494728297009932 23701
0.499485255733384 23801
0.496129539211154 23901
0.491753862259904 24001
0.483236305639732 24101
0.471011999719693 24201
0.454969971637582 24301
0.433455349875856 24401
0.40547893297672 24501
0.369128347073396 24601
0.322751735491683 24701
0.263125545578124 24801
0.18380365272952 24901
0.0738907203112626 25001
0 25101
0 25201
0 25301
0 25401
0 25501
0 25601
0 25701
0 25801
0 25901
0 26000
}{\GroupLasso}


==> data/heatmap.tex <==










